Algorithmic Strategies for Sustainable Reuse of Neural Network Accelerators with Permanent Faults

Hardware failures are a growing challenge for machine learning accelerators, many of which are based on systolic arrays. When a permanent hardware failure occurs in a systolic array, existing solutions include localizing and isolating the faulty processing element (PE), using a redundant PE for re-execution, or in some extreme cases decommissioning the entire accelerator for further investigation. In this paper, we propose novel algorithmic approaches that mitigate permanent hardware faults in neural network (NN) accelerators by uniquely integrating the behavior of the faulty component instead of bypassing it. In doing so, we aim for a more sustainable use of the accelerator where faulty hardware is neither bypassed nor discarded, instead being given a second life. We first introduce a CUDA-accelerated systolic array simulator in PyTorch, which enabled us to quantify the impact of permanent faults appearing on links connecting two PEs or in weight registers, where one bit is stuck at 0 or 1 in the float32, float16, or bfloat16 representation. We then propose several algorithmic mitigation techniques for a subset of stuck-at faults, such as Invertible Scaling or Shifting of activations and weights, or fine tuning with the faulty behavior. Notably, the proposed techniques do not require any hardware modification, instead relying on existing components of widely used systolic array based accelerators, such as normalization, activation, and storage units. Extensive experimental evaluations using fully connected and convolutional NNs trained on MNIST, CIFAR-10 and ImageNet show that the proposed fault-tolerant approach matches or gets very close to the original fault-free accuracy.

==> Dump/algorithmic.tex <==
\textcolor{blue}{Similarly, to calculate $c$ for faulty bit position $p$ in the float16 exponent range, we follow that:
\begin{itemize}
    \item If the affected bit position $14 \geq p \geq 11$:
    \begin{equation}
    \label{c-bit-11-to-14}
        c = 2^{E - 15}, \;\;\;\;\;\; \mbox{where } E = \sum_{i=10}^{p - 1} 2^{i-10}
    \end{equation}
    \item If the affected bit position $p = 10$:
    \begin{equation}
    \label{c-bit-10}
    c = 2^{-14} \times \sum_{i=1}^{10}2^{-i}
    \end{equation}
\end{itemize}
}

\textcolor{blue}{Finally, to calculate $c$ for faulty bit position $p$ in the bfloat16 exponent range, we follow that:
\begin{itemize}
    \item If the affected bit position $14 \geq p \geq 8$:
    \begin{equation}
    \label{c-bit-8-to-14}
        c = 2^{E - 127}, \;\;\;\;\;\; \mbox{where } E = \sum_{i=7}^{p - 1} 2^{i-7}
    \end{equation}
    \item If the affected bit position $p = 7$:
    \begin{equation}
    \label{c-bit-7}
    c = 2^{-126} \times \sum_{i=1}^{7}2^{-i}
    \end{equation}
\end{itemize}
}

==> Dump/characterization.tex <==
\subsubsection*{\textcolor{blue}{Mantissa stuck-at faults}}\label{sec:mantissa_faults}

\textcolor{blue}{With the exception of down link faults, we observed that stuck-at faults in the mantissa range had negligible impact on performance across all fault type  x data type x model x dataset combinations, with an average relative error increase (REI) of $< 1\%$ as shown in Figures ~\ref{fig:all-models-float16-fi}, ~\ref{fig:all-models-bfloat16-fi} and ~\ref{fig:all-models-float32-fi}  In general, the most significant mantissa bit positions had the greatest impact on test accuracy.}
\textcolor{blue}{For the FCN using the MNIST dataset, we observed that the effect of the fault was more pronounced for reduced precision mantissa fields across the different data types.
For example, the average REI for down link stuck-at-1 faults for float32, float16 and bfloat16 were $7.33\%$, $7.64\%$ and $7.95\%$ respectively.}
\textcolor{blue}{In contrast among the CNNs (LeNet, AlexNet, and VGG16), the float16 data type had negligible impact on performance for down link stuck-at-1 faults with a REI $< 1\%$. The shallower CNNs (LeNet and AlexNet) exhibited an improvement in performance when switching from the float32 to bfloat16 data type. LeNet’s average REI for down link stuck-at-1 fault in the most significant bit decreased from $10.33\%$ to $2.60\%$, likewise AlexNet’s average REI also decreased from $1.65\%$ to $0.72\%$, suggesting reduced precision mantissa fields may be more tolerant for worst case mantissa stuck-at faults for smaller networks. Networks with increased depth and greater number of parameters such as VGG16 showed less variation of performance impact across all data types.
Given the most significant mantissa bit stuck-at fault were among the worst affected across all data types, we focus our efforts on mitigating them.}

\subsubsection*{\textcolor{blue}{Exponent stuck-at-1 faults}}\label{sec:exp_sb1_faults}

\textcolor{blue}{Right link faults indicated degrading performance as the affected bits ranged from least to most significant.}
\textcolor{blue}{It is interesting to observe in Figures ~\ref{fig:all-models-float16-fi}, ~\ref{fig:all-models-bfloat16-fi} and ~\ref{fig:all-models-float32-fi} that for the FCN, we see oscillation in terms of performance for down link faults. While the 3 most significant exponent bits exhibit worsening performance degradation as the significance of the bit position increases across all data types, the exponent bits following show the opposite effect, until a sharp drop at the most significant exponent bit with an average REI of $1068.39\%$ for both float16 and bfloat16 and $1042.99\%$ for float32. A similar trend is observed for weight register faults, though to a reduced degree of severity as the effect of the fault is localized to the faulty PE and thus only its partial sum contribution to the output of the systolic array.}
\textcolor{blue}{In the case of CNNs, the oscillating behavior of performance degradation for down link and weight register faults is dampened signficantly as the model increases in depth and number of parameters across all data types as shown in Figures ~\ref{fig:all-models-float16-fi}, ~\ref{fig:all-models-bfloat16-fi} and ~\ref{fig:all-models-float32-fi}. The sharp drop in performance at the most significant bit position remains, and can be seen as worse for deeper networks such as AlexNet and VGG16 than compared to LeNet. In the case of AlexNet and VGG16 the sharp drop is approximately the same across all fault types for any floating point representation. For instance in the case of float32,  AlexNet and VGG16 both exhibited a consistent average REI of ~$133$ and ~$266\%$ across all link and weight register faults respectively.}

\subsubsection*{\textcolor{blue}{Exponent stuck-at-0 faults}}\label{sec:exp_sb0_faults}

\textcolor{blue}{Right link faults had negligible drop in performance for most cases (REI $<1\%$) as shown in Figures ~\ref{fig:all-models-float16-fi} to ~\ref{fig:all-models-float32-fi}. The exceptions were in the case of the most significant bit for the FCN, which saw an average REI of $89.97\%$, $90.45\%$ and $78.36\%$ for float16, bfloat16 and float32 respectively, and bit positions 24 to 29 for VGG16 using the float32 data type which saw slight degradation in performance with an average REI between 2.08 to 7.27\%. Compared to exponent stuck-at-1 faults, we observe minimal impact. This is likely due to exponent bits already being zero due to the normalization of weights and activations before passing through the first layer of the NN, minimizing the effect of stuck-at-0 faults in the exponent range. }
\textcolor{blue}{Down link faults showed more stable decrease in performance than their stuck-at-1 counterparts for the FCN with the worst case average REI of 104.21\%, 105.15\% and 104.54\% for float16, bfloat16 and float32 respectively. The CNNs (LeNet, AlexNet, VGG16) had a higher tolerance to down link faults as shown in Figures ~\ref{fig:all-models-float16-fi} to ~\ref{fig:all-models-float32-fi}, with the same trend for performance observed across the exponent bit range as described in Section ~\ref{sec:characterization} It is interesting to note that the float32 data type was more affected than compared to float16 and bfloat16. Considering float32 and bfloat16 both share the same number of bits in the exponent field, it is possible that the reduced precision in the mantissa range of the bfloat16 format acts as a form of regularization, by restricting the range of a value that can be represented thus preventing large deviations.}
\textcolor{blue}{The FCN and LeNet both had their parameters initialized using Kaiming uniform distribution before training. The minimal impact on performance for weight register faults may be attributed to the bounded range of values of this initialization scheme, $\mathcal{U}(-bound, bound)$, where $bound =\sqrt{\frac{3}{|f_{in}|}}$ and $f_{in}$ is the number of input nodes in the linear layer ~\cite{PyTorchKaimingUniformInit}, by setting a number of exponent bit positions to zero by default.
Deeper networks (AlexNet, VGG16) had a lower average REI across all exponent bit positions as observed in Figures ~\ref{fig:all-models-float16-fi}, ~\ref{fig:all-models-bfloat16-fi} and ~\ref{fig:all-models-float32-fi}, fault and data types. This may be attributed to higher level layers being able to compensate for lower level layers by capturing high level features of an image, and the over parameterization of the networks allowing affected neurons to have less impact on the overall classification. }

\subsubsection*{\textcolor{blue}{Sign stuck-at faults}}\label{sec:sign_faults}

\textcolor{blue}{Right link stuck-at faults had negligible drop in performance across all models. In the case of the FCN, the ReLU activation function between layers helped to ensure activation values in subsequent layers were positive, reducing the effect of sign bit stuck-at-0 faults. Weight register faults also had limited impact as shown in Figures ~\ref{fig:all-models-float16-fi} to ~\ref{fig:all-models-float32-fi}, given their effect is limited to the partial sum contribution of the affected PE and can be compensated by healthy PEs in the affected column within the systolic array.
The worst performing sign bit faults were attributed to down link stuck-at-0 faults particularly for larger models such as AlexNet and VGG16 using float32. Reduced precision data types such as float16 and bfloat16 appear to be more tolerant to stuck-at sign bit faults, likely due to smaller deviations from the expected fault free values as shown in Figures 7 to 9.}



% \subsubsection*{\textcolor{blue}{Fully Connected Network} on MNIST}\label{mnist_char}
% \textcolor{blue}{Using the MNIST dataset, we trained a 2 hidden layer FCN as shown in Figure 5, which achieved an original fault-free test accuracy of $92.3\%$. The model was trained and tested using a $8 \times 8$ WS systolic array.}

% \textcolor{blue}{$\rightarrow$ \textit{Mantissa stuck-at faults:}
% Throughout testing, we observed that on average, stuck-at faults in the mantissa range had negligible impact on performance across all fault and data types, with an average relative error increase (REI) of $<1\%$ as shown in Figures ~\ref{fig:all-models-float16-fi}, ~\ref{fig:all-models-bfloat16-fi} and ~\ref{fig:all-models-float32-fi}. The largest REI was noted for the two most significant mantissa bit positions. As the number of bits dedicated to represent the mantissa decreased across the different data types, the REI increased for link faults. For instance, for down link faults in the most signficant mantissa bit position, the REI for float32, float16 and bfloat16 were $7.33\%$, $7.64\%$ and $7.95\%$ respectively. This may be attributed to the reduced precision of the mantissa range. Therefore, we concentrate our efforts on mitigating the most significant mantissa bit positions.}

% \textcolor{blue}{$\rightarrow$ \textit{Exponent stuck-at-1 faults:} Right link faults indicated degrading performance as the affected bits ranged from least to most significant. It is interesting to observe that for down link faults we see oscillation in terms of performance. While the 3 least significant exponent bits for all data types exhibited worsening performance degradation as the significance of the bit position increased, the exponent bits following showed the opposite effect, until a sharp drop at the most significant exponent bit, which contributed to a REI of $1068.39\%$ for both float16 and bfloat16 and $1042.99\%$ for float32 data types. A similar trend was observed for weight register faults, though to a reduced degree of severity as the effect of the fault is localised to the faulty PE and only its partial sum contribution to the output, assuming all unaffected PEs have their weights loaded correctly.}

% \textcolor{blue}{$\rightarrow$ \textit{Exponent stuck-at-0 faults:}
% Right link faults had a negligible drop in performance except for the most significant exponent bit which had a REI of $89.97\%$, $90.45\%$ and $78.36\%$ for float16, bfloat16 and float32 respectively. The most significant exponent bit is likely to already be zero for activation values due to normalization, as such this type of fault is less severe. Down link faults showed more stable decrease in performance than compared to exponent stuck-at-1 faults, with the worst case REI of $104.21\%$, $105.15\%$ and $104.54\%$ for float16, bfloat16 and float32 respectively.
% Weight register faults had little to no impact, likely due to the use of Kaiming uniform distribution used to initialize the weights between the bound of $\sqrt{\frac{3}{|f_{in}|}}$, where $f_{in}$ is the number of input nodes in the linear layer ~\cite{PyTorchKaimingUniformInit}, thereby setting the bit positions within the exponent range to zero.}

% \textcolor{blue}{$\rightarrow$ \textit{Sign stuck-at faults:} Right link stuck-at-0 faults had negligible impact on performance, likely due to the use of ReLU activation functions between layers ensuring activation values in subsequent layers within the FCN were positive, however stuck-at-1 faults saw a REI of $397.26\%$, $398.22\%$ and $346.67\%$ across the float16, bfloat16 and float32 data types. Down link stuck-at-0 faults had almost 3 times REI on test accuracy across all data types than compared to their stuck-at-1 counterparts. In contrast weight register stuck-at-1 faults had almost 1.7 and 1.9 times REI on performance for float16/bfloat16, and float32 data types respectively.}





==> Dump/cuda.tex <==
\subsection{High-Performance S3A for fault injection using CUDA}

\textcolor{purple}{RCB: In case we need space, this subsection will either be compressed considerably or eliminated and moved into an Appendix later ...}

\textcolor{blue}{This section outlines the implementation of a Systolic Array-like Matrix Multiplication (SMM) algorithm using CUDA to enhance computational efficiency in order to solve the some limitations of standard S3A \ref{sec:limitations}. Our approach leverages CUDA's parallel processing capabilities to accelerate this fundamental operation.\\
To inject faults that mimic a fault within a systolic array, it is essential to understand the data dependencies and what can be processed independently.}


%DO NOT USE THIS FIG FOR PAPER MUST REWORK
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{Figures/SmmFig.jpg}
    \caption{\textcolor{blue}{This figure shows an example of how tiled matrix multiplication. The input matrix has dimensions \( N \times M \), the weight matrix has dimensions \( M \times O \), and the resulting output matrix has dimensions \( N \times O \). To tile, both matrices are divided into smaller tiles of size \( d \times d \) corresponding to the dimension of the systolic array.}}
    \label{fig:tiledMM}
\end{figure}

\textcolor{blue}{At the core of systolic array multiplication is tiling. The weight and input tiles are loaded into the array and processed through the system. In the figure \ref{fig:tiledMM}, we illustrate the process of computing the final output tile (purple) in a matrix multiplication operation using tiled matrices. Each input (highlighted in green) is multiplied by the corresponding weight tile (highlighted in blue). These multiplications produce partial products, which are then accumulated (summed) to form the final output tile in matrix \( C \) (highlighted in purple).\\ %MAKE A FIG FOR DESCRIBING THE RESULTANT 5D MATRIX
To accurately model the impact of faults on the partial sums transmitted on down links and accumulated in output registers, it is crucial to keep output tiles separated before summing them. The resultant is defined as a 5D tensor. It is best conceptualized as having dimensions: (number of column tiles in the output, number of row tiles in the output, the number of partial sum output tiles, dimension of systolic array, dimension of systolic array). To better understand this, imagine the third dimension as a list containing \( d \times d \) subtiles.}

\begin{algorithm}[h]
    \centering
    \caption{Systolic Matrix Multiplication Kernel}
    \begin{algorithmic}
        \Require $InputTensor$, $WeightTensor$, $OutputTensor$, $n$, $m$, $o$, $d$
        \State $i \gets \text{blockIdx.x} \times \text{blockDim.x} + \text{threadIdx.x}$
        \State $j \gets \text{blockIdx.y} \times \text{blockDim.y} + \text{threadIdx.y}$
        \If{$i < n$ \textbf{and} $j < o$}
            \For{$k = 0$ \textbf{to} $m-1$}
                \State $input \gets InputTensor[i][k]$
                \State $weight \gets WeightTensor[k][j]$
                \State $partial\_sum \gets OutputTensor[i/d][j/d][k/d][i\%d][j\%d]$
                \State Apply fault to $input$, $weight$, or $partial\_sum$ based on fault type
                \State $OutputTensor[i/d][j/d][k/d][i\%d][j\%d] \gets input \times weight + partial\_sum$
            \EndFor
        \EndIf
    \end{algorithmic}
    \label{sudo:smmKernel}
\end{algorithm}

\textcolor{blue}{To calculate the output matrix, we collapse the third dimension by adding the partial sum output tiles together, yielding the output tiles, which are then flattened to form the final matrix.
To parallelize the tile computation effectively and leverage CUDA's multiprocessing capabilities, we need to parallelize the matrix multiplication of the tiles while maintaining the cascading effects of faults.
Right links are the easiest dependency to break. To determine if the input data sent through the right link is impacted by a fault, we need to check if the data is used after passing through a faulty right link or register. Down links are slightly more challenging. However, since we store the partial sums accumulated sequentially within their correct positions but separately from other partially accumulated sums in the output subtiles, we need to inject the fault once based on its occurrence during accumulation. Both cases can be managed by indexing the correct positions using modular arithmetic.}





%add sudocode here
 

\textcolor{blue}{This CUDA-based implementation utilizes a systolic array for efficient parallel matrix multiplication and includes mechanisms for injecting faults into the computation process. This approach ensures both high performance and robustness in matrix operations.
}

%RCB: Put w and a in Figure 1 to connect with w and a in figure 4.

%RCB: What is the speed-up over the simple PyTorch implementaiton in terms of M, N, d, ... which for the CNN on ImageNet meant from 2 .5 days to 3 hours.

\textcolor{blue}{The computational complexity of the vanilla S3A algorithm is O$\left(\left\lceil \frac{N}{d} \right\rceil \times \left\lceil \frac{M}{d} \right\rceil \times \left\lceil \frac{O}{d} \right\rceil \times d\right)$ whereas the complexity of the CUDA implementation is O$\left(m\right)$ with the appropriate GPU resources. This reduction in time complexity results in significant time improvements for deeper networks, reducing computation time from approximately 2.5 days to 2 hours.}

==> Dump/fc-ber.tex <==

\textcolor{blue}{\subsection{Fault Combinations (FC) and Bit Error Rate (BER) Analysis}}\label{sec:fault-combo-ber}

\textcolor{blue}{In addition to single stuck-at faults in any link or weight register within a systolic array, our techniques can also be extended to handle a combination of faults, as follows:}
\textcolor{blue}{\begin{itemize}
    \item \textbf{FC1:} Multiple stuck-at-0 \textit{or} stuck-at-1 faults in the exponent field, can be mitigated using ISc or ISc + Flip respectively, by modifying the calculation of the constant used to scale values in Section VI-A Step 2, by selecting p as the least significant faulty stuck bit position. For example, if bit positions 24, 26-29 were stuck-at-0 for float32, we select p to be 24. This ensures that all affected bit positions have their value set to 0 when passing through the fault, rendering its effect inconsequential. 
    \item \textbf{FC2:} Multiple stuck-at-0 \textit{or} stuck-at-1 faults in the sign bit position within down links or weight registers within a single column of PEs can be mitigated using IScSh. The same holds for right link faults where multiple stuck-at-0 \textit{or} stuck-at-1 faults occur within a single row of PEs by utilizing IScSh + Trp. This assumes that a single column (or row in the case of right link stuck-at faults) contains only a single fault type, either stuck-at-0 or stuck-at-1.
    \item \textbf{FC3:} Combination of stuck-at-0 and/or stuck-at-1 faults in the sign bit position across a number of columns (in the case of down link and weight register faults), or rows (in the case right link faults) can be mitigated using IScSh or IScSh + Trp. This also assumes that any affected column (or row in the case of right link stuck-at faults) contains only a single fault type, either stuck-at-0 or stuck-at-1.
\end{itemize}}

\textcolor{blue}{The fault configurations which are not supported include a combination:}
\textcolor{blue}{\begin{itemize}
    \item \textbf{FC4:} Multiple stuck-at-0 \textit{and} stuck-at-1 faults in the exponent field within the same link or weight register. In this case, a constant to scale the values as specified in Section VI-A Step 2 cannot be reliably calculated as stuck-at-1 faults require the flipped exponent representation, that will incorrectly calculate values in the presence of already existing stuck-at-0 faults.
    \item \textbf{FC5:} Combination of stuck-at-0 \textit{and} stuck-at-1 faults in the sign bit position within the same column (for down link and weight register faults) or row (for right link faults) of PEs cannot reliably use IScSh as the preloaded partial sum value in the top PE cannot guarantee partial sum values stay within the range of either positive or negative values that match the affected sign bit position.
\end{itemize}}

\textcolor{blue}{The maximum BER that can be accommodated for the aforementioned faults depends on the size of the systolic array as well as the floating point data type used. These are presented in Tables ~\ref{tab:link_ber_table} and ~\ref{tab:wr_ber_table} for link and register faults respectively. The tolerable BER for weight register faults is double that of link faults as the number of right and down links is double that of weight registers in any $d \times d$ systolic array.}
\begin{table}
    \centering
    \caption{\textcolor{blue}{Maximum Mitigated BER for Right and Down Link Fault Combinations (FC), Across Systolic Array Dimensions ($d$) and Data Types.}}
    \label{tab:link_ber_table}
    \begin{tabular}{|*{5}{c|}}
    \hline
    & \textcolor{blue}{$d$} & \textcolor{blue}{\textbf{float16}} & \textcolor{blue}{\textbf{bfloat16}}  & \textcolor{blue}{\textbf{float32}}
    \\
     \hline
    \multirow{4}{4em}{\textcolor{blue}{\textbf{Single SB 0 or 1}}} & \textcolor{blue}{8} & \multicolumn{2}{|c|}{\textcolor{blue}{$4.88 \times 10^{-4}$}} & \textcolor{blue}{$2.44 \times 10^{-4}$}
    \\ 
    & \textcolor{blue}{64} & \multicolumn{2}{|c|}{\textcolor{blue}{$7.63 \times 10^{-6}$}} & \textcolor{blue}{$3.81 \times 10^{-6}$} \\ 
    & \textcolor{blue}{128} & \multicolumn{2}{|c|}{\textcolor{blue}{$1.91 \times 10^{-6}$}}& \textcolor{blue}{$9.54 \times 10^{-7}$} \\ 
    & \textcolor{blue}{256} & \multicolumn{2}{|c|}{\textcolor{blue}{$4.77 \times 10^{-7}$}} & \textcolor{blue}{${2.38  \times 10^{-7}}$} \\ 
    \hline
    \multirow{4}{4em}{\textcolor{blue}{\textbf{FC1}}} & \textcolor{blue}{8} & \textcolor{blue}{$2.44 \times 10^{-3}$} & \textcolor{blue}{$ 3.9 \times 10^{-3}$} & \textcolor{blue}{$1.95 \times 10^{-3}$} 
    \\ 
    & \textcolor{blue}{64} & \textcolor{blue}{$3.82 \times 10^{-5}$} & \textcolor{blue}{$6.10 \times 10^{-5}$} & \textcolor{blue}{$3.05 \times 10^{-5}$} \\ 
    & \textcolor{blue}{128} & \textcolor{blue}{$9.55 \times 10^{-6}$} & \textcolor{blue}{$1.53 \times 10^{-5}$} & \textcolor{blue}{$1.95 \times 10^{-3}$} \\ 
    & \textcolor{blue}{256} & \textcolor{blue}{$2.39 \times 10^{-6}$} & \textcolor{blue}{$3.82 \times 10^{-6}$} & \textcolor{blue}{$1.9 \times 10^{-6}$} \\ 
    \hline
    \multirow{4}{4em}{\textcolor{blue}{\textbf{FC2}}} & \textcolor{blue}{8} & \multicolumn{2}{|c|}{\textcolor{blue}{$3.9 \times 10^{-3}$}} & \textcolor{blue}{$1.95 \times 10^{-3}$} 
    \\ 
    & \textcolor{blue}{64} & \multicolumn{2}{|c|}{\textcolor{blue}{$4.88 \times 10^{-4}$}} & \textcolor{blue}{$2.44 \times 10^{-4}$} \\ 
    & \textcolor{blue}{128} & \multicolumn{2}{|c|}{\textcolor{blue}{$2.44 \times 10^{-4}$}} & \textcolor{blue}{$1.22 \times 10^{-4}$} \\ 
    & \textcolor{blue}{256} & \multicolumn{2}{|c|}{\textcolor{blue}{$1.22 \times 10^{-4}$}} & \textcolor{blue}{$6.1 \times 10^{-5}$} \\ 
    \hline
    \multirow{4}{4em}{\textcolor{blue}{\textbf{FC3}}} & \textcolor{blue}{8} & \multicolumn{2}{|c|}{\textcolor{blue}{$3.12 \times 10^{-2}$}} & \textcolor{blue}{$1.56 \times 10^{-2}$} 
    \\ 
    & \textcolor{blue}{64} & \multicolumn{2}{|c|}{\textcolor{blue}{$3.13 \times 10^{-2}$}} & \textcolor{blue}{$1.56 \times 10^{-2}$} \\ 
    & \textcolor{blue}{128} & \multicolumn{2}{|c|}{\textcolor{blue}{$3.13 \times 10^{-2}$}} & \textcolor{blue}{$1.56 \times 10^{-2}$} \\ 
    & \textcolor{blue}{256} & \multicolumn{2}{|c|}{\textcolor{blue}{$3.13 \times 10^{-2}$}} & \textcolor{blue}{$1.56 \times 10^{-2}$} \\ 
    \hline
    \end{tabular}
\end{table}

\begin{table}
    \centering
    \caption{\textcolor{blue}{Maximum Mitigated BER for Register Fault Combinations (FC), Across Systolic Array Dimensions ($d$) and Data Types.}}
    \label{tab:wr_ber_table}
    \begin{tabular}{|*{5}{c|}}
    \hline
    & \textcolor{blue}{$d$} & \textcolor{blue}{\textbf{float16}} & \textcolor{blue}{\textbf{bfloat16}}  & \textcolor{blue}{\textbf{float32}}  
    \\
     \hline
    \multirow{4}{4em}{\textcolor{blue}{\textbf{Single SB 0 or 1}}} & \textcolor{blue}{8} & \multicolumn{2}{|c|}{\textcolor{blue}{$9.77 \times 10^{-4}$}} & \textcolor{blue}{$4.88 \times 10^{-4}$}
    \\ 
    & \textcolor{blue}{64} & \multicolumn{2}{|c|}{\textcolor{blue}{$1.53 \times 10^{-5}$}} & \textcolor{blue}{$7.63 \times 10^{-6}$} \\ 
    & \textcolor{blue}{128} & \multicolumn{2}{|c|}{\textcolor{blue}{$3.81 \times 10^{-6}$}}& \textcolor{blue}{$1.91 \times 10^{-6}$} \\ 
    & \textcolor{blue}{256} & \multicolumn{2}{|c|}{\textcolor{blue}{$9.54 \times 10^{-7}$}} & \textcolor{blue}{${4.77 \times 10^{-7}}$} \\ 
    \hline
    \multirow{4}{4em}{\textcolor{blue}{\textbf{FC1}}} & \textcolor{blue}{8} & \textcolor{blue}{$4.89 \times 10^{-3}$} & \textcolor{blue}{$7.82 \times 10^{-3}$} & \textcolor{blue}{$3.9 \times 10^{-3}$} 
    \\ 
    & \textcolor{blue}{64} & \textcolor{blue}{$7.65 \times 10^{-5}$} & \textcolor{blue}{$1.22 \times 10^{-4}$} & \textcolor{blue}{$6.1 \times 10^{-5}$} \\ 
    & \textcolor{blue}{128} & \textcolor{blue}{$1.91 \times 10^{-5}$} & \textcolor{blue}{$3.0 \times 10^{-4}$} & \textcolor{blue}{$1.53 \times 10^{-5}$} \\ 
    & \textcolor{blue}{256} & \textcolor{blue}{$4.77 \times 10^{-6}$} & \textcolor{blue}{$7.63 \times 10^{-6}$} & \textcolor{blue}{$3.82 \times 10^{-6}$} \\ 
    \hline
    \multirow{4}{4em}{\textcolor{blue}{\textbf{FC2}}} & \textcolor{blue}{8} & \multicolumn{2}{|c|}{\textcolor{blue}{$7.82 \times 10^{-3}$}} & \textcolor{blue}{$3.9 \times 10^{-3}$} 
    \\ 
    & \textcolor{blue}{64} & \multicolumn{2}{|c|}{\textcolor{blue}{$9.79 \times 10^{-4}$}} & \textcolor{blue}{$4.88 \times 10^{-4}$} \\ 
    & \textcolor{blue}{128} & \multicolumn{2}{|c|}{\textcolor{blue}{$4.88 \times 10^{-4}$}} & \textcolor{blue}{$2.44 \times 10^{-4}$} \\ 
    & \textcolor{blue}{256} & \multicolumn{2}{|c|}{\textcolor{blue}{$2.44 \times 10^{-4}$}} & \textcolor{blue}{$1.22 \times 10^{-4}$} \\ 
    \hline
    \multirow{4}{4em}{\textcolor{blue}{\textbf{FC3}}} & \textcolor{blue}{8} & \multicolumn{2}{|c|}{\textcolor{blue}{$6.25 \times 10^{-2}$}} & \textcolor{blue}{$3.12 \times 10^{-2}$} 
    \\ 
    & \textcolor{blue}{64} & \multicolumn{2}{|c|}{\textcolor{blue}{$6.27 \times 10^{-2}$}} & \textcolor{blue}{$3.13 \times 10^{-2}$} \\ 
    & \textcolor{blue}{128} & \multicolumn{2}{|c|}{\textcolor{blue}{$6.24 \times 10^{-2}$}} & \textcolor{blue}{$3.13 \times 10^{-2}$} \\ 
    & \textcolor{blue}{256} & \multicolumn{2}{|c|}{\textcolor{blue}{$6.25 \times 10^{-2}$}} & \textcolor{blue}{$3.13 \times 10^{-2}$} \\ 
    \hline
    \end{tabular}
\end{table}


